Extending DeepSDF for automatic 3D shape retrieval and similarity transform estimation

Recent advances in computer graphics and computer vision have found successful application of deep neural network models for 3D shapes based on signed distance functions (SDFs) that are useful for shape representation, retrieval, and completion. However, this approach has been limited by the need to have query shapes in the same canonical scale and pose as those observed during training, restricting its effectiveness on real world scenes. We present a formulation to overcome this issue by jointly estimating shape and similarity transform parameters. We conduct experiments to demonstrate the effectiveness of this formulation on synthetic and real datasets and report favorable comparisons to the state of the art. Finally, we also emphasize the viability of this approach as a form of 3D model compression.

==> sections/metrics.tex <==
\subsection{Metrics}\label{sec:metrics}
We have made use of the F-score as recommended in \cite{tatarchenko2019single} to provide a quantitative evaluation of our work. Given a groundtruth shape $S$ and an estimate shape $\hat{S}$, as well as samples of points on their surfaces $\partial \Omega_{S}^{\phantom{-}},\partial \Omega_{\hat{S}}^{\phantom{-}} $\footnote{For simplicity, we have retained the same notation as that used for the set of all points on the surface. To compute the F-score, we can only use a sampling of the set of points on the surface.} the F-score is the harmonic mean of precision and recall metrics. Precision and recall are defined as follows: 

To compute the precision, for each point in the estimate shape, we first compute its distance to the groundtruth as:
\begin{equation*}
    e_{y} = \underset{x \in \partial \Omega_{S}^{\phantom{-}}}{\text{min}} || y - x||_2
\end{equation*}

The precision is then computed as the percentage of points within distances less than $\epsilon_{p}$.
\begin{equation}
    P(\epsilon_p) = \frac{100}{|\partial \Omega_{\hat{S}}^{\phantom{-}}|} \sum_{y \in \partial \Omega_{\hat{S}}^{\phantom{-}}} \mathbf{1}_{\{e_{y} < \epsilon_{p}\}}
\end{equation}

Recall is computed in the opposite direction.  Again, the error is first computed as:
\begin{equation}
    e_{x} = \underset{y \in \partial \Omega_{\hat{S}}^{\phantom{-}}}{\text{min}} || x - y||_2
\end{equation}
and recall as:
\begin{equation}
     R(\epsilon_r) = \frac{100}{|\partial \Omega_{S}^{\phantom{-}}|}\sum_{x \in \partial \Omega_{S}^{\phantom{-}}} \mathbf{1}_{\{e_{x} < \epsilon_{r}\}}
\end{equation}
Finally, the F-score is computed as:
\begin{equation}
    F(\epsilon) = \frac{2P(\epsilon)R(\epsilon)}{P(\epsilon) + R(\epsilon)}
\end{equation} 
The F-score ranges from 0 to 1, with higher values indicating a better match between the estimate and the groundtruth. The F-score is very sensitive to deviations in shape and thus makes an excellent metric. To obtain pointclouds from the meshes, we have sampled 3000 points from the surface of each mesh. We have also set $\epsilon = 0.05r$, where $r$ is the radius of the bounding sphere of the shape $S$. 

An alternative metric may have been computing the distance between the estimated parameters and the groundtruth parameters, however, we find that solutions that are close in 3D space may not be close in the metric space. For example, we find that the learned shapes have slightly different centers from their groundtruth counterparts, as such a good result may have a different translation value than the groundtruth. The exception to this is the rotation since all the learned shapes face the same direction. In our experiments, we assume the axis of rotation is known and report the error in the angle of rotation about this axis $|\hat{\theta} - \theta|$. 

